Think Globally, Act Locally: A Deep Neural Network Approach to High-Dimensional Time Series Forecasting

Forecasting high-dimensional time series plays a crucial role in many applications such as demand forecasting and financial predictions. Modern datasets can have millions of correlated time-series that evolve together, i.e they are extremely high dimensional (one dimension for each individual time-series). There is a need for exploiting global patterns and coupling them with local calibration for better prediction. However, most recent deep learning approaches in the literature are one-dimensional, i.e, even though they are trained on the whole dataset, during prediction, the future forecast for a single dimension mainly depends on past values from the same dimension. In this paper, we seek to correct this deficiency and propose DeepGLO, a deep forecasting model which thinks globally and acts locally. In particular, DeepGLO is a hybrid model that combines a global matrix factorization model regularized by a temporal convolution network, along with another temporal network that can capture local properties of each time-series and associated covariates. Our model can be trained effectively on high-dimensional but diverse time series, where different time series can have vastly different scales, without a priori normalization or rescaling. Empirical results demonstrate that DeepGLO can outperform state-of-the-art approaches; for example, we see more than 25% improvement in WAPE over other methods on a public dataset that contains more than 100K-dimensional time series.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
Time-series forecasting is a core machine learning problem that plays a key role in automating business processes across the industry~\cite{larson2001designing}. For instance, in the retail industry demand forecasting requires predicting the future demand for a large number of products based on past data. The number of products can range in millions, and thus one needs to forecast a large number of correlated time-series (one for each product). Such a setting is often referred to as high-dimensional multivariate time-series forecasting~\cite{seeger2016bayesian,yu2016temporal}.

Traditional time-series forecasting methods operate on individual time-series or a small number of time-series at a time. These methods include the well known AR, ARIMA and exponential smoothing~\cite{mckenzie1984general}, the classical Box-Jenkins methodology~\cite{box1968some} and more generally the linear state-space models~\cite{hyndman2008forecasting}. However, these methods suffer from a few main drawbacks when it comes to forecasting high-dimensional multi-variate time-series data: 

{\bf (C1)} They are trained on individual time-series and cannot benefit from training on large datasets.

{\bf (C2)} Most of these models are linear and cannot learn non-linear patterns in the data.

{\bf (C3)} As during training, these models predict time-series individually  and cannot leverage information from other correlated time-series evolving together, during prediction.

Deep networks have been gaining in popularity in time-series forecasting in recent times and can potentially address some of the issues mentioned above. Recurrent Neural Networks (RNN's)~\cite{funahashi1993approximation} have been popular in sequential modeling, however they suffer from the gradient vanishing/exploding problems in training. Long Short Term Memory (LSTM)~\cite{gers1999learning} networks alleviate that issue and have had great success in langulage modeling and other seq-to-seq tasks~\cite{gers1999learning,sundermeyer2012lstm}. Recently, deep time-series models have used LSTM blocks as internal components~\cite{flunkert2017deepar,rangapuram2018deep}. Another popular architecture, that is competitive with LSTM's and easier to train are temporal convolutions/causal convolutions popularized by the wavenet model~\cite{van2016wavenet}. Temporal convolutions have been recently used in time-series forecasting~\cite{borovykh2017conditional,bai2018empirical}. These models can be trained on the whole dataset and can learn non-linear dependencies (handling {\bf (C1),(C2)}). However, {\bf (C3)} is still a concern as these models only work on individual time-series during prediction. Moreover, these deep models lead to another concern,

{\bf (C4)} These deep models have difficulty training on data-sets with wide variations in scale among time-series and need a priori normalization during training. This can lead to loss of accuracy as explained in Section~\ref{sec:leveled} and~\ref{sec:results}. Such variations in scale are common, for instance in retail some products may have much higher demands than others.

In~\cite{lai2018modeling}, the authors propose a combination of 2D convolution and recurrent connections, that can take in multiple time-series in the input layer thus also handling {\bf (C3)} in addition to {\bf (C1),(C2)}. However, this method does not scale more than a few thousand time-series. On the other end of the spectrum, TRMF~\cite{yu2016temporal} is a temporally regularized matrix factorization model that can express all the time-series as linear combinations of \textit{basis time-series}. This model can handle the issues {\bf (C1),(C3)} and {\bf(C4)}, however lacks expressive power because of the linearity assumption ({\bf (C4)}).

In this paper we aim to propose a model that can alleviate all the above shortcomings {\bf (C1)-(C4)}. The \textit{main contributions} of this paper are as follows,

{\bf (i)} In Section~\ref{sec:leveled}, we propose a variation of of the temporal convolution architecture called the \textit{leveled network} that can be trained effectively on data-sets with wide scale variations, \textit{without} a priori normalization. Thus this model can handle {\bf (C1),(C2)(C4)}, but still only focuses on individual time-series during prediction.

{\bf (ii)} Then in Section~\ref{sec:trmf}, inspired by TRMF~\cite{yu2016temporal}, we introduce Deep Temporal Matrix Factorization (DTRMF) which can express each time-series as linear combination of $k$ basis time-series, where $k$ is much less than the number of time-series. Unlike TRMF, this model can capture non-linear dependencies as the regularization and prediction is done using a leveled network trained concurrently. This model can handle {\bf (C1)-(C4)} as the basis time-series can capture global dependencies while prediction.

{\bf (iii)} In Section~\ref{sec:hybrid}, we combine the DTRMF model proposed with a leveled network trained on the original data-set, through a linear attention model. This leads to a stronger model that focuses on both local properties on individual time-series and global dependencies in the data-set while training and prediction. This model is termed as the Hybrid DTRMF model.

{\bf (iv)} Finally, in Section~\ref{sec:results}, we show that our models outperform other benchmarks on three real world time-series data-set: electricity~\cite{elec} [370 time-series], traffic~\cite{cuturi2011fast} [960 time-series] and wiki~\cite{wiki} [111k time-series], in the context of rolling predictions.




  

==> pdef.tex <==
\section{Problem Setting}
\label{sec:pdef}

We consider the problem of forecasting high-dimensional time series over future time-steps. High-dimensional time-series datasets consist of several possibly correlated time-series evolving over time and the task is to forecast the values of those time-series in future time-steps. Before, we formally define the problem, we will set up some notation. 

{\bf \noindent Notation: }  We will use bold capital letters to denote matrices such as $\*Y \in \-R^{m \times n}$. $Y_{ij}$ denotes the $(i,j)$-th entry of the matrix $\*Y$. Let $[n] \triangleq \{1,2,...,n\}$ for a positive integer $n$. Any subset $\Omega \subseteq [m] \times [n]$ can be used to denote a set of indices of the matrix $\*Y$. In the special case where $\Omega = \{m_1,...,m_r\}  \times \{n_1,...,n_c\} $, $\*Y_{\Omega}$ denotes the sub-matrix comprising of the entries. When $\Omega = \{m_1,...,m_r\}  \times \{n_1,...,n_c\} $ and $n_1,...,n_c$ are contiguous, $\Omega^{(1)}$ will be used to denote the set of indices $\{m_1,...,m_r\}  \times \{n_1+1,...,n_c+1\}$ i.e the column indices shifted by $1$. Sub-matrices consisting of continuous indices will be denoted as $\*Y_{i:i+r,s:s+c} \triangleq \*Y_{\Omega}$, where $\Omega = [i,i+1,...,i+r]\times[s,s+1,...,s+c]$. $\norm{\*Y}_F$, $\norm{\*Y}_2$ denote the Frobenius and Spectral norms respectively. $\norm{\*x}_p$ denotes the $p$-norm of the vector $\*x$. $\*x_{\_A}$ denotes the sub-vector with entries $\{x_i : \forall i \in \_A\}$ where $x_i$ denotes the $i$-th coordinate of $\*x$ and $\_A \subseteq [n]$. The notation $\*x_{i:j}$ will be used to denote the vector $[x_i,...,x_j]$. The notation $[\*x;\*y]$ will be used to denote the concatenation of the vectors $\*x$ and $\*y$. for a vector $\*x \in \-R^{n}$, $\mu(\*x) \triangleq (\sum_i x_i) / n$ denotes the empirical mean of the coordinates and $\sigma(\*x) \triangleq \sqrt{(\sum_i (x_i - \mu(\*x)^2)) / n }$ denotes the empirical standard deviation. 

{\bf Forecasting Task: } A time-series data-set can be represented by a matrix $\*Y \in \-R^{n \times t}$ where $n$  is the number of time-series, each with $t$ time-points. $\Omega_{tr} = [n] \times \{1,2,...,t-\tau\}$ denotes the training indices, that is $\*Y_{\Omega_{tr}}$ is the observed training matrix. $\Omega_{te} = [n] \times \{t-\tau+1,...,t\}$ denotes the test indices, that is $\*Y_{\Omega_{tr}}$ is the test range which needs to be predicted. $\hat{\*Y}_{\Omega_{te}}$ will be used to denote the predicted values in the test range by a forecasting model under consideration, given the observed values $\*Y_{\Omega_{tr}}$. The $i$-th time series will be denoted by the $t$ dimensional row vector $\*y^{(i)}$, which represents the $i$-th row of $\*Y$.

{\bf Objective: } The quality of the predictions are generally measured using a loss function between the predicted and actual values in the test range. One of the popular loss metric is the normalized absolute deviation metric~\cite{yu2016temporal}, defined as follows,
\begin{align}
\label{eq:metric}
\_L(\hat{\*Y},\*Y) = \frac{\sum_{i = 1}^{n'}\sum_{j=1}^{t'} |Y_{ij} - \hat{Y}_{ij}|}{\sum_{i = 1}^{n'}\sum_{j=1}^{t'} |Y_{ij} |},
\end{align}
where $\*Y \in \-R^{n'\times t'}$ represents the actual values while  $\hat{\*Y} \in \-R^{n'\times t'}$ are the corresponding predictions. This metric is often referred to as WAPE in the forecasting literature. Other commonly used loss metrics are define in Section~\ref{sec:metric}.

==> temporal.tex <==
\section{Temporal Building Blocks}
\label{sec:temporal}
Traditionally in the deep learning literature, time-series models are based on recurrent architectures~\cite{flunkert2017deepar,rangapuram2018deep}. The most commonly used base architecture is the Long Short Term Memory (LSTM)~\cite{gers1999learning} recurrent networks. However, in more recent works it has been observed that sequence-sequence tasks can be effectively performed by dilated Temporal Convolution architectures (popularized by the Wavenet model~\cite{van2016wavenet}). In addition Temporal Convolutions are more stable while training and can provide competitive or better performance as compared to recurrent models~\cite{bai2018empirical}. Therefore, in this work we will use Temporal Convolution (TC) blocks as the basic building blocks for our prediction models. We provide a brief description of TC in the next section, for the sake of completeness. 
\subsection{Temporal Convolution}
\label{sec:leveled}
Temporal convolution (also referred to as Causal Convolution)~\cite{van2016wavenet,borovykh2017conditional,bai2018empirical} are multi-layered neural networks comprised of 1D convolutional layers. The major difference from regular 1D convolution, is the introduction of \textit{dilation} in the filter taps, which guarantees a much larger dynamic range. Dilation is equivalent to introducing a fixed step between every two adjacent
filter taps. The dilation in layer $i$ is usually set as $d(i) = 2^{i-1}$. A temporal convolution network with filter size $k$ and number of layers $r$ has a dynamic range (or look-back) of $l = 1 + 2(k-1)2^{r-1}$. An example of a temporal convolution network with one channel per layer is shown in Fig.~\ref{fig:conv}. TC networks can also have residual connections as shown in Fig.~\ref{fig:conv}. For more details, we refer the readers to the general description in~\cite{bai2018empirical}. Note that in practice, we can have multiple channels per layer of a TC network. 

\begin{figure}[h!]
	\centering
	\includegraphics[width=\linewidth]{TCN.pdf}
	\caption{Illustration of a TC network with zero-padding to confirm to input shape. The network has $r=4$ layers, with filter size $k=3$ and number of channels $1$ in each layer. It also has a residual connection as shown. The network maps the input $\*y_{0:t-1}$ to the one-shifted output $\hat{\*y}_{1:t}$.}
	\label{fig:conv}
\end{figure}

Thus, the temporal convolution network can be treated as an object that takes in the previous values of a time-series $\*y_{t-l+1:t}$ and outputs the one-step look ahead predicted values $\hat{\*y}_{t-l+2:t+1}$. We will denote neural network functions as calligraphic capital letters. Thus given a TC network $\_T(\cdot)$, we can write $\hat{\*y}_{t-l+2:t+1} = \_T(\*y_{t-l+1:t})$. We will use the notation $\_T^{(p)}(\cdot)$ to denote the value of the last time-step predicted by the TC network $\_T()$, i.e $\hat{y}_{t+1} = \_T^{(p)}(\*y_{t-l+1:t})$. The same operators can be defined on matrices. Given $\*Y \in \-R^{n \times t}$ and a set of indices $\Omega = \{i_1,...,i_{n'}\} \times \{s,s+1,...,s + l - 1\}$ such that $i_j \in [n]$ and $\{s,s+1,...,s + l - 1\} \subset [t]$ we can write $\hat{\*Y}_{\Omega^{(1)}} = \_T(\*Y_{\Omega})$. Thus, $\Omega^{(1)}$ represents the one-step shifted indices $\{i_1,...,i_{n'}\} \times \{s+1,...,s + l\}$. With some abuse of notation, $\_T(\*y_{t-l+1:t};W)$ will be used to denote operation of the TC network on a sequence, where the network weights are $W$. The network weights $W$ are updated during training. %Temporal Convolution networks can be trained using mini-batches that consist of consecutive time-steps and can be used to make multi-step future predictions as detailed in the subsequent sections. 

\subsection{Leveled Network - Handling Diverse Scales}
Large scale time-series datasets containing upwards of hundreds of thousands of time-series can have very diverse scales. The diversity in scale leads to issues in training deep models, both Temporal Convolutions and LSTM based architectures, and some normalization is needed for training to succeed~\cite{lai2018modeling,borovykh2017conditional,flunkert2017deepar}. However, selecting the correct normalizing factor for each time-series is not an exact science and can have effects on predictive performance. For instance in~\cite{flunkert2017deepar} the data-sets are whitened using the training standard deviation and mean of each time-series while training, and the predictions are renormalized. On the other hand in~\cite{borovykh2017conditional}, each time-series is rescaled by the value of that time-series on the first time-step. Moreover, when performing rolling predictions using a pre-trained model, when new data is observed there is a potential need for updating the scaling factors by incorporating the new time-points. In this section we propose a simple \textit{leveling network} architecture that can be trained on diverse datasets without the need for a priori normalization.

The \textit{leveled network} architecture consists of two temporal convolution blocks (having the same dynamic range $l$) that are trained concurrently. Let us denote the two networks and the associated weights by $\_T_a(;W_a)$ and $\_T_m(;W_m)$ respectively. The key idea is to have $\_T_m(;W_m)$ (the leveling component) predict the rolling mean of the next $w$ future time-points given the past ($w$ is termed as the window size). On the other-hand $\_T_a(;W_a)$ (the additive component) will be used to predict the variations around this mean value. Given an appropriate window size the rolling mean stays stable for each time-series and can be predicted by a simple temporal convolution model and given these predictions the additive variations are relatively scale free i.e. the network $\_T_a(;W_a)$ can be trained reliably without normalization. This can be summarized by the following equations,
\begin{align*}
\hat{a}_{t+1} &= \_T^{(p)}_a(\*y_{t-l+1:t})\\
\hat{m}_{t+1} &= \_T^{(p)}_m(\*y_{t-l+1:t}), \numberthis \label{eq:leveled}
\end{align*}
where we want $\hat{m}_{t+1}$ to be close to $\mu(\*y_{t:t+w-1})$ and $\hat{a}_{t+1}$ to be close to $y_t - \mu(\*y_{t:t+w-1})$. An illustration of the leveled network methodology is shown in Fig.~\ref{fig:leveled}.

{\bf \noindent Training:} Both the networks can be trained concurrently given the training set $\*Y_{\Omega_{tr}}$, using mini-batch stochastic gradient updates. The pseudo-code for the training process has been provided as Algorithm~\ref{algo:TCtrain}. In Algorithm~\ref{algo:TCtrain}, the loss function $\_L(.,.)$ used is the same as the metric defined in Eq.~\eqref{eq:metric}. Note that in Step 9, the leveling component $\_T_m(;W_m)$ is held fixed and only $\_T_a(;W_a)$ is updated.

\begin{algorithm}                      
	\caption{Training the Leveled Network}          
	\label{algo:TCtrain}  
	\small                         
	\begin{algorithmic}[1]   
		\STATE {\bf Arguments}: Number of epochs: $n_e$, Horizontal batch-size: $t_b$, Vertical batch-size: $n_b$, Learning rate: $\eta$, Window size: $w$.      
		\STATE Initialize $\_T_a(;W_a)$ and $\_T_m(;W_m)$; $n = 1$
		\WHILE {$n \leq n_e$}
		\WHILE {End of Epoch is reached}
		\STATE Get mini-batch $\Omega = \{i_1,...,i_{n_b}\} \times \{s,s+1,...,s + t_b - 1\}$ (concurrent time-indices)
		\STATE Let $\hat{\*A}_{\Omega^{(1)}} = \_T_a(\*Y_{\Omega};W_a)$ and $\hat{\*M}_{\Omega^{(1)}} = \_T_m(\*Y_{\Omega};W_m)$. 
		\STATE Let $\*M_{\Omega^{(1)}}$ be the matrix such that the $(r,c)$-th entry is $\mu(\*y^{(i_r)}_{s+c:s+c+w})$.
		\STATE $W_m = W_m -\eta \frac{\partial}{W_m} \_L(\hat{\*M}_{\Omega^{(1)}}, \*M_{\Omega^{(1)}})$
		\STATE $W_a = W_a -\eta \frac{\partial}{W_a} \_L(\hat{\*A}_{\Omega^{(1)}}+\hat{\*M}_{\Omega^{(1)}}, \*Y_{\Omega^{(1)}})$
		\ENDWHILE
		\STATE $n = n + 1$.
		\ENDWHILE
	\end{algorithmic}
\end{algorithm}

\begin{figure}[h!]
	\centering
	\includegraphics[width = 0.8\linewidth]{leveled.pdf}
	\caption{\small Illustration of the leveled network. The leveling component $\hat{m}^{(i)}_{t+1}$ and the additive component $\hat{a}^{(i)}_{t+1}$ are predicted as functions of the past $\*y^{(i)}_{t-l+1:t}$. The final prediction is  $\hat{m}^{(i)}_{t+1} + \hat{a}^{(i)}_{t+1}$.}
	\label{fig:leveled}
\end{figure}

{\bf \noindent Prediction:} The trained model can be used for multi-step look-ahead prediction in a standard manner. Given the past data-points of a time-series, $\*y_{t-l+1:t}$, the prediction for the next time-step is given by, $\hat{y}_{t+1} = \_T^{(p)}_a(\*y_{t-l+1:t}) + \_T^{(p)}_m(\*y_{t-l+1:t})$. Now, the one-step look-ahead prediction can be concatenated with the past values to form the sequence $\tilde{\*y}_{t-l+2:t+1} = [\*y_{t-l+1:t};\hat{y}_{t+1}]$ and then again passed through the two networks to yield $\hat{y}_{t+2} = \_T^{(p)}_a(\tilde{\*y}_{t-l+2:t+1}) + \_T^{(p)}_m(\tilde{\*y}_{t-l+2:t+1})$. This can be repeated $k$ times to predict $k$ time-steps into the future. Henceforth, a leveled temporal convolution block $\_T() = \_T_m() + \_T_a()$ will be denoted by a calligraphic capital letter as a whole (for instance $\_T$). 

In Section~\ref{sec:results}, we shall see that the \textit{leveled network} can be trained on unnormalized data-sets with wide variations in scale. In the next section, we introduce our hybrid model, \golf, in which the leveled network is used as internal components both in the global and local parts of the model.

==> trmf.tex <==
\section{Matrix Factorization Regularized by Leveled Network - The Global Model}
\label{sec:trmf}
In this section we propose a low-rank matrix factorization model for time-series forecasting that uses a leveled network for regularization. This approach is inspired by the Temporally Regularized Matrix Factorization (TRMF) model in~\cite{yu2016temporal}. 

\begin{figure}[h!]
	\centering
	\includegraphics[width=\linewidth]{trmf_illustrate.pdf}
	\caption{Illustration of the matrix factorization approach in time-series forecasting. The $\*Y_{\Omega_{tr}}$ training matrix can be factorized into low-rank factors $\*F$ ($\in \- R^{n \times k}$) and $\*X^{(tr)}$ ($\in \-R ^{k \times (t - \tau)}$). If the $\*X^{(tr)}$ preserves temporal structures then the future values $\*X^{(te)}$ can be predicted by a time-series forecasting model and thus the test period predictions can be made as $\*F\*X^{(tr)}$.}
	\label{fig:factors}
\end{figure}

The idea is to factorize the training time-series matrix $\*Y_{\Omega_{tr}}$ into low-rank factors $\*F$ ($\in \-R^{n \times k}$) and $\*X^{(tr)}$ ($\in \-R^{k \times (t - \tau)}$), where $k \ll n$. This is illustrated in Fig.~\ref{fig:factors}. Further, we would like the $\*X_{tr}$ matrix to have temporal structure, such that the future values $\*X^{(te)}$ in the test range can be predicted. Let $\*X = [\*X^{(tr)};\*X^{(te)}]$ Thus, the matrix $\*X$ can be thought of to be comprised of $k$ \textit{basis time-series} that capture the global temporal patterns in the whole data-set and all the original time-series are linear combinations of these basis time-series. In the next subsection we will describe how such a temporal structure can be encouraged using a concurrently trained leveled network. 

{\bf Regularization Through Leveled Network: } If we are provided with a leveled network that captures the temporal patterns in the training data-set $\*Y_{\Omega_{tr}}$, then we can encourage temporal structures in $\*X^{(tr)}$ using this model. Let us assume that the said leveled network is $\_T_X(.)$. The temporal patterns can be encouraged by ensuring that the temporal loss, 
\begin{equation}
\label{eq:temporal_loss}
\_L_{T}(\*X^{(tr)};\_T_X(.)) = \sum_{s=l}^{t-\tau}\frac{ \_L\left(\*X^{(tr)}_{1:n,s} , \_T^{(p)}_{X}(\*X^{(tr)}_{1:n,s-l:s-1}\right)}{t-\tau-l+1}
\end{equation}
is minimized, where $\_L(.,.)$ is the metric defined in Eq.~\ref{eq:metric}. This implies that the values of the $\*X^{(tr)}$ on time-index $s$ are close to the predictions from the temporal network applied on the past values between time-steps $\{s-l,...,s-1\}$. Here, $l$ is ideally equal to the dynamic range of the network defined in Section~\ref{sec:temporal}. Thus the overall loss function for the factors and the temporal network is given by,
\begin{equation}
\label{eq:global_loss}
\_L_G(\*F,\*X^{(tr)},\_T_X) = \_L\left(\*F\*X^{(tr)},\*Y_{\Omega_{tr}}  \right)+ \lambda_{\_T} \_L(\*X^{(tr)};\_T_X(.)),
\end{equation}
where $\lambda_{\_T}$ is the regularization hyper-parameter. 

\begin{algorithm}[!ht]                      
	\caption{Training the Low-rank factors $\*F,\*X^{(tr)}$ given a fixed network $\_T_X(.)$, for one epoch}          
	\label{algo:factors}                           
	\begin{algorithmic}[1]   
		\STATE Arguments: Horizontal batch-size: $t_b$, Vertical batch-size: $n_b$, Learning rate: $\eta$  
		\WHILE {End of Epoch is reached}
		\STATE Get next mini-batch: $\Omega = \{n',n'+1,...,n'+n_b-1\}\times\{t',t'+1,...,t'+t_b-1\}$.
		\STATE Let \begin{align*}L &= \_L\left( \*F\*X_{1:k,t':t'+t_b-1},\*Y_{\Omega}\right) \\&+ \lambda_{\_T}\_L\left( \*X_{1:k,t':t'+t_b-1},\_T_X(\*X_{1:k,t'-1:t'+t_b-2})\right)\end{align*}
		\STATE Update \[\*F_{n':n'+n_b-1,1:k} = \*F_{n':n'+n_b-1,1:k} - \frac{\eta\partial L}{\partial\*F_{n':n'+n_b-1,1:k}}.\]
		\STATE Update \[\*X_{1:k,t':t'+t_b-1} =  \*X_{1:k,t':t'+t_b-1}  - \frac{\eta\partial L}{\partial\*X_{1:k,t':t'+t_b-1} }.\]
		\ENDWHILE   
	\end{algorithmic}
\end{algorithm}

{\bf Training:} The low-rank factors $\*F,\*X^{(tr)}$ and the temporal network $\_T_X(.)$ can be trained alternatively to minimize the loss in Eq.~\eqref{eq:global_loss}. The overall training can be performed through mini-batch SGD and can be broken down into two main components performed alternately: $(i)$ given a fixed $\_T_X(.)$ approximately minimize $\_L_G(\*F,\*X^{(tr)},\_T_X)$ with respect to the factors $\*F,\*X^{(tr)}$ - Algorithm~\ref{algo:factors} and $(ii)$ train the network $\_T_X(.)$ on the matrix $\*X^{(tr)}$ using Algorithm~\ref{algo:TCtrain}. 

The overall algorithm is detailed as Algorithm~\ref{algo:dtrmf}. The leveled network is first initialized on a normalized version of the data-set. Here, by normalized we mead that each time-series is centered and scaled by the empirical mean and standard deviation of the said time-series in the training range. Note that this does not imply that the remaining training is done on the normalized data-set. Then in the second initialization step, the factors are trained using the initialized $\_T_X(.)$ (step 4), for $n_s$ epochs. This is followed by the alternative training (steps 6-9). 

\begin{algorithm}[!ht]                      
	\caption{Deep Temporal Matrix factorization (DTRMF)}          
	\label{algo:dtrmf}                           
	\begin{algorithmic}[1]   
		\STATE Arguments: Horizontal batch-size: $t_b$, Vertical batch-size: $n_b$, Learning rate: $\eta$, \#Seeding epochs: $n_s$, \#Training epochs: $n_t$, Number of alternate runs: $n_a$. 
		\STATE{// {\em Initialize model training}} 
		\STATE Initialize $\_T_X()$ by training it on a normalized version of $\*Y_{\Omega_{tr}}$, using Algorithm~\ref{algo:TCtrain} for $n_s$ epochs/ till early stop.
		\STATE Train the factors for $n_s$ epochs using Algorithm~\ref{algo:factors}. 
		\STATE {// {\em Alternate training cycles}}
		\FOR {$i = 1,2,...,n_a$}
		\STATE Train the factors for $n_t$ epochs/early stop using Algorithm~\ref{algo:factors}.
		\STATE Train  $\_T_X()$ on $\*X^{tr}$ using Algorithm~\ref{algo:TCtrain} for $n_t$ epochs/ till early stop.
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

{\bf Rolling Prediction:} Once the model is trained using Algorithm~\ref{algo:dtrmf}, we can make predictions on the test range using multi-step look-ahead prediction. The method is straight-forward - we first use $\_T_X(.)$ to make multi-step look-ahead prediction on the basis time-series in $\*X^{(tr)}$ as detailed in Section~\ref{sec:temporal}, to obtained $\hat{\*X}^{(te)}$; then the original time-series predictions can be obtained by $\hat{\*Y}_{\Omega_{te}} = \*F\hat{\*X}^{(te)}$.

This model can also be adapted to make rolling predictions \textit{without retraining}. In the case of rolling predictions, the task is to train the model on the training period say $\*Y_{1:n,1:t_1}$, then make predictions on a future time period say $\hat{\*Y}_{1:n,t_1+1:t_2}$, then receive the actual values on the future time-range $\*Y_{1:n,t_1+1:t_2}$ and after incorporating these values make further predictions for a time range further in the future $\hat{\*Y}_{1:n,t_2+1:t_3}$ and so on. The key challenge in this scenario, is to incorporate the newly observed values $\*Y_{1:n,t_1+1:t_2}$ to generate the values of the basis time-series in that period that is $\*X_{1:k,t_1+1:t_2}$. We obtain these new values through minimizing a hybrid loss function. First we predict these values using the trained network $\_T_X$ and the past factor matrix $\*X_{1:k,1:t_1}$, to obtained $\hat{\*X}_{1:k,t_1+1:t_2}$. Then, we obtain the $\*X_{1:k,t_1+1:t_2}$ by minimizing the following loss,
\begin{align*}
\*X_{1:k,t_1+1:t_2} &= \argmin_{\*X \in \-R^{k \times (t_2-t_1)}} (1 - \alpha)\_L\left(\*F\*X,\*Y_{1:n,t_1+1:t_2}\right) \\
&+ \alpha \_L(\*X,\hat{\*X}_{1:k,t_1+1:t_2}),
\end{align*}
where $\_L$ is the metric defined in Eq.~\eqref{eq:metric} and $\alpha \in (0,1)$ is a hyper-parameter. The first part of the loss encourages $\*F\*X$ to be close to the newly revealed values $\*Y_{1:n,t_1+1:t_2}$ and the second part encourages $\*X$ to have temporal structures as predicted by the leveled network. Once we obtain $\*X_{1:k,t_1+1:t_2}$, we can make predictions in the next set of future time-periods $\hat{\*Y}_{1:n,t_2+1:t_3}$. Note that the TRMF model in~\cite{yu2016temporal} needed to be retrained from scratch to incorporate the newly observed values. In this work retraining is not required to achieve good performance, as we shall see in our experiments in Section~\ref{sec:results}. We set $\alpha = 0.2$ in all our experiments.

\section{Hybrid DTRMF: Local and Global Models}
\label{sec:hybrid}
In Section~\ref{sec:trmf}, we introduced the DTRMF model that can leverage global information from the whole data-set even during prediction time, through the linear combinations of the basis time-series. In this section, we will extend that model to leverage both global information (through basis time-series in DTRMF) and local information (through a separate leveled network $\_T_Y()$ that is trained on the original data-set and predicts the future values of each time-series based on its past). The final output is through a linear attention model that combines the global and local predictions. 

\begin{algorithm}[!ht]                      
	\caption{Hybrid DTRMF: Local and Global models}          
	\label{algo:complete}                           
	\begin{algorithmic}[1]   
		\STATE Train DTRMF model on the training data-set using Algorithm~\ref{algo:dtrmf}.
		\STATE Train local leveled network $\_T_Y$ on the original time-series $\*Y_{\Omega_{tr}}$ using Algorithm~\ref{algo:TCtrain}. Set $n=1$.
		\STATE  {// {\em Training attention model}}
		\WHILE {$n \leq n_e$}
		\WHILE {End of Epoch is reached}
		\STATE Get mini-batch $\Omega = \{i_1,...,i_{n_b}\} \times \{s,s+1,...,s + t_b - 1\}$ (concurrent time-indices)
		\STATE Let $\hat{\*A}_{\Omega^{(1)}}^{(g)},\hat{\*A}_{\Omega^{(1)}}^{(l)} = \_T_A(\*Y_{\Omega};W_A)$ 
		\STATE $\hat{\*Y}^{(g)}_{\Omega^{(1)}} = \*F\*X_{1:k,s:s+t_b-1}$.
		\STATE $\hat{\*Y}^{(a)}_{\Omega^{(1)}} = \_T_Y(\*Y_{\Omega})$.
		\STATE $W_A = W_A -\eta \frac{\partial}{W_A} \_L(\hat{\*Y}^{(g)}_{\Omega^{(1)}}*\hat{\*A}_{\Omega^{(1)}}^{(g)} + \hat{\*Y}^{(l)}_{\Omega^{(1)}}*\hat{\*A}_{\Omega^{(1)}}^{(l)}, \*Y_{\Omega^{(1)}})$
		\ENDWHILE
		\STATE $n = n + 1$.
		\ENDWHILE
	\end{algorithmic}
\end{algorithm}

The idea is to have a simple temporal convolution network $\_T_A$ that outputs attention weights based on the past values of a time series $\*y^{(i)}_{1:s}$. These attention weights are used to combine local and global predictions. For the sake of exposition, we will write the relations for one step look-ahead predictions, 
\begin{align*}
&\hat{\*X}_{1:k,s+1} = \_T_X^{(p)}(\*X_{1:k,s-l:s})\\
&\hat{\*Y}^{(g)}_{1:n,s+1} = \*F\hat{\*X}_{1:k,s+1} ~~\text{(global DTRMF prediction)} \\
&\hat{\*A}^{(g)}_{1:n,s+1},\hat{\*A}^{(l)}_{1:n,s+1} =  \_T_A^{(p)}(\*Y_{1:k,s-l:s})
 ~~\text{(attention weights)}\\
&\hat{\*Y}^{(l)}_{1:n,s+1} = \_T_Y^{(p)}(\*Y_{1:n,s-l:s}) ~~\text{(local predictions)}\\
&\hat{\*Y}_{1:n,s+1} = \hat{\*Y}^{(g)}_{1:k,s+1}*\hat{\*A}^{(g)}_{1:n,s+1} \\
&+ \hat{\*Y}^{(l)}_{1:k,s+1}*\hat{\*A}^{(l)}_{1:n,s+1} ~~\text{(hybrid predictions)},
\end{align*}
where '*' means element-wise multiplication. 

Thus the final predictions are linear combinations of the local and global predictions. The linear attention weights are predicted by a temporal convolution network $ \_T_A()$ based on the past values of the time-series. This network can be trained by mini-batch SGD as detailed in our complete algorithm in Algorithm~\ref{algo:complete}. Steps 1 and 2 involve training the global DTRMF model and the locally focused leveled network $\_T_Y()$ on the original data-set. Steps 5-12 provides the pseudo-code for training the attention TC $\_T_A()$.

Note that rolling predictions and multi-step predictions can be performed by the hybrid model, as the individual global DTRMF model and the local leveled network $\_T_Y$ can perform the same independently, without any need for re-training.






==> trmfv3.tex <==
\section{\golf: A Deep Global Local Forecaster}
\label{sec:deepglo}
In this section, we propose \golf, our complete hybrid model which
consists of separate global and local components, married through a
data-driven attention mechanism. In Section~\ref{sec:trmf}, we present the
global component, Deep Leveled Network regularized Matrix Factorization  (\MFLN). This model can capture global patterns
during prediction, by representing each of the original time-series as a
linear combination of $k$ basis time-series, where $k \ll n$. The local model
is simply a \dln trained on the original dataset. In
Section~\ref{sec:hybrid}, we detail how the global and local models are
combined.

\begin{minipage}{0.43\textwidth}
	\vspace{-1em}
	\begin{algorithm}[H]
		\caption{Mini-batch Training for \dln}
		\label{algo:TCtrain}
		\scriptsize
		\begin{algorithmic}[1]
			\Require {learning rate $\eta$, horizontal batch size $b_t$, vertical
				batch size $b_n$, window size $w$, and $\texttt{maxiters}$}
			%\STATE {\bf Arguments}: Number of epochs: $n_e$, Horizontal batch-size: $t_b$, Vertical batch-size: $n_b$, Learning rate: $\eta$, Window size: $w$.
			\State Initialize $\Theta_r$ and $\Theta_m$
			\For {$\texttt{iter} = 1, \cdots, \texttt{maxiters}$}
			\For {each batch with indices $\cI$ and $\cJ$ in an epoch}
			\State $\cI = \cbr{i_1,...,i_{b_n}}$ and $\cJ = \cbr{j+1,j+2,...,j + b_t}$
			\State $\*M \leftarrow \texttt{mean}\cbr{\*Y[\cI, \cJ + s]: s = 1, \cdots, w}$
			\State
			%\begin{align*}
			$\hat{\*M} \leftarrow \cT_m(\*Y[\cI,\cJ]|\Theta_m)$ and $\hat{\*R} = \cT_r(\*Y[\cI,\cJ]|\Theta_r)$\\
			%\end{align*}
			\State $\Theta_m \leftarrow \Theta_m -\eta \frac{\partial}{\Theta_m} \_L(\*M, \hat{\*M})$
			\State
			$\Theta_r \leftarrow \Theta_r -\eta \frac{\partial}{\Theta_r} \_L(\*Y[I, J + 1], \hat{\*M} + \hat{\*R})$
			\EndFor
			\EndFor
		\end{algorithmic}
	\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.43\textwidth}
	\begin{algorithm}[H]
		\caption{\golf - Deep Global Local Forecaster}
		\label{algo:factors}
		\scriptsize
		\begin{algorithmic}[1]
			\Require \texttt{maxiters}
			%\STATE Train \MFLN model on the training data-set using Algorithm~\ref{algo:dtrmf}.
			\State Obtain global $\*F$, $\Xtr$ and $\cT_X(\cdot)$ by Alg~\ref{algo:dtrmf}.
			\State Obtain local \dln $\cT_Y(\cdot)$ by Alg~\ref{algo:TCtrain} on $\Ytr$.
			\State  {/* {\em Training attention model} */ }
			\For {$\texttt{iter} = 1,\ldots, \texttt{maxiters}$}
			\For {each batch with indices $\cI$ and $\cJ$}
			\State $\cI = \cbr{i_1,...,i_{b_n}}$ and $\cJ =  \cbr{s,s+1,...,s + b_t - 1}$.
			\State Let $\hat{\*A}^{(g)},\hat{\*A}^{(l)} = \cT_A(\*Y[\cI,\cJ-1]|\Theta_A)$
			\State $\hat{\*Y}^{(g)} = \*F[\cI,:]\*X[:, \cJ]$.
			\State $\hat{\*Y}^{(l)} = \cT_Y(\*Y[\cI, \cJ - 1])$.
			\State Let $\hat{\*Y} = \hat{\*Y}^{(g)}\odot\hat{\*A}^{(g)} + \hat{\*Y}^{(l)}\odot\hat{\*A}^{(l)}$
			\State
			$\Theta_A = \Theta_A -\eta \frac{\partial}{\Theta_A} \_L(\*Y[\_I,\cJ], \hat{\*Y})$
			\EndFor
			\EndFor
		\end{algorithmic}
	\end{algorithm}
	
	\vspace{-1em}
\end{minipage}

\subsection{Global: Deep Leveled Network regularized Matrix Factorization (\MFLN)}
\label{sec:trmf}
In this section we propose a low-rank matrix factorization model for
time-series forecasting that uses a leveled network for regularization. 
The idea is to factorize the training time-series matrix $\Ytr$ into low-rank
factors $\*F\in \-R^{n \times k}$ and $\Xtr \in \-R^{k \times t}$,
where $k \ll n$. This is illustrated in Figure~\ref{fig:factors}. Further, we
would like to encourage a temporal structure in $\Xtr$ matrix, such that the
future values $\Xte$ in the test range can also be forecasted. Let
$\*X = [\Xtr \Xte]$ Thus, the matrix $\*X$ can be thought of to be
comprised of $k$ \textit{basis time-series} that capture the global temporal
patterns in the whole data-set and all the original time-series are linear
combinations of these basis time-series. In the next subsection we will
describe how a \dln can be used to encourage the temporal structure for $\*X$.

{\bf Temporal Regularization by a \dln:} If we are provided with a leveled
network that captures the temporal patterns in the training data-set
$\Ytr$, then we can encourage temporal structures in $\Xtr$ using
this model. Let us assume that the said leveled network is $\_T_X(\cdot)$. The
temporal patterns can be encouraged by including the following temporal
regularization into the objective function:
\begin{align}
&\_R(\Xtr\mid \_T_X(\cdot)) := \frac{1}{|\cJ|}\_L\rbr{\*X[:,\cJ],
\cT_{X}\rbr{\*X[:, \cJ - 1]}},\label{eq:temporal_loss}
%&:= \sum_{s=l}^{t-\tau}\frac{ \_L\left(\*X^{(tr)}[:,s] , \_T^{(p)}_{X}(\*X^{(tr)}[:,s-l:s-1])\right)}{t-\tau-l+1} \numberthis
\end{align}
where $\cJ = \cbr{l, \cdots, t}$ and $\_L(\cdot,\cdot)$ is the metric defined
in Eq.~\eqref{eq:metric}. This implies that the values of the $\*X^{(tr)}$ on
time-index $j$ are close to the predictions from the temporal network applied
on the past values between time-steps $\{j-l,...,j-1\}$. Here, $l$ is ideally
equal to the dynamic range of the network defined in
Section~\ref{sec:temporal}. Thus the overall loss function for the factors and
the temporal network is as follows:
\begin{align}
  \cL_G(\Ytr,\*F,\Xtr,\cT_X)
  := \cL\rbr{\Ytr, \*F\Xtr} + \lambda_{\cT} \cR(\Xtr \mid \cT_X(\cdot)), \label{eq:global_loss}
\end{align}
where $\lambda_{\_T}$ is the regularization parameter for the temporal
regularization component.



{\bf Training:} The low-rank factors $\*F,\Xtr$ and the temporal network
$\cT_X(\cdot)$ can be trained alternatively to approximately minimize the loss
in Eq.~\eqref{eq:global_loss}. The overall training can be performed through
mini-batch SGD and can be broken down into two main components performed
alternatively: $(i)$ given a fixed $\cT_X(\cdot)$ approximately minimize
$\cL_G(\*F,\Xtr,\cT_X)$ with respect to the factors $\*F,\Xtr$ -
Algorithm~\ref{algo:factors} and $(ii)$ train the network $\cT_X(\cdot)$ on
the matrix $\Xtr$ using Algorithm~\ref{algo:TCtrain}.

The overall algorithm is detailed in Algorithm~\ref{algo:dtrmf}. The global
\dln $\cT_X(\cdot)$ is first initialized by training on a normalized version
of $\Ytr$. Here, by normalized we mean that each dimension of the time-series
is centered and scaled by the empirical mean and standard deviation of the
same dimension of time-series in the training range. Note that this normalized
$\Ytr$ is only used to initialize $\cT_X(\cdot)$. Then in
the second initialization step, two factors $\*F$ and $\Xtr$
are trained using the initialized $\cT_X(\cdot)$ (step 3), for
$\texttt{iters}_{\texttt{init}}$ iterations.
This is followed by the $\texttt{iters}_{\texttt{alt}}$ alternative steps to
update $\*F$, $\Xtr$, and $\cT_X(\cdot)$ (steps 5-7).

\begin{remark}
Note that \MFLN can perform rolling predictions without retraining unlike \trmf. We provide more details in Appendix~\ref{sec:roll}, in the interest of space.
\end{remark}

\begin{minipage}{0.43\textwidth}
	
	
	
	\begin{algorithm}[H]
		\caption{Temporal Matrix Factorization Regularized by Leveled Network (\MFLN)}
		\label{algo:dtrmf}
		\scriptsize
		\begin{algorithmic}[1]
			\Require $\texttt{iters}_{\texttt{init}}$, $\texttt{iters}_{\texttt{train}}$, $\texttt{iters}_{\texttt{alt}}$.
			\State {/* {\em Model Initialization} */}
			\State Initialize $\cT_X(\cdot) $ by Alg~\ref{algo:TCtrain} on a normalized version of $\Ytr$ for $\texttt{iters}_{\texttt{init}}$ iterations.
			\State Initialize $\*F$ and $\Xtr$ by Alg~\ref{algo:factors} for $\texttt{iters}_{\texttt{init}}$ iterations.
			\State {/* {\em Alternate training cycles} */}
			\For {$\texttt{iter} = 1,2,...,\texttt{iters}_{\texttt{alt}}$}
			\State Update $\*F$ and $\Xtr$ by Alg~\ref{algo:factors} for $\texttt{iters}_{\texttt{train}}$ iterations
			\State Update $\cT_X(\cdot)$ by Alg~\ref{algo:TCtrain} on $\Xtr$ for $\texttt{iters}_{\texttt{train}}$ iterations
			\EndFor
		\end{algorithmic}
	\end{algorithm}
	
\end{minipage}
\hfill
\begin{minipage}{0.43\textwidth}
	
	
	\begin{algorithm}[H]
		\caption{ Training the Low-rank factors $\*F,\Xtr$ given a fixed network $\_T_X(\cdot)$, for one epoch }
		\label{algo:complete}
		\scriptsize
\begin{algorithmic}[1]
	\Require learning rate $\eta$, a \dln model $\cT_X(\cdot)$.% horizontal batch size $b_t$, vertical batch size $b_n$
	\For {each batch with indices $\cI$ and $\cJ$ in an epoch}
	\State $\cI = \cbr{i_1,...,i_{b_n}}$ and $\cJ = \cbr{j+1,j+2,...,j + b_t}$
	%\STATE Let \begin{align*}L &= \_L\left( \*F[\_I,:]\*X[:,\_J],\*Y[\_I,\_J]\right) + \lambda_{\_T}\_R\left( \*X[:,\_J] \mid \_T_X()\right)\end{align*}
	\State $\*X[:,\cJ] \leftarrow \*X[:,\cJ]  -\eta \frac{\partial}{\partial\*X[:,\cJ]} \cL_G(\*Y[\cI,\cJ],\*F[\cI,:], \*X[:, \cJ], \cT_X)$
	\State $\*F[\cI,:] \leftarrow \*F[\cI,:] - \eta \frac{\partial}{\partial\*F[\cI,:]} \cL_G(\*Y[\cI,\cJ],\*F[\cI,:], \*X[:, \cJ], \cT_X)$
	\EndFor
\end{algorithmic}
\end{algorithm}
	%\vspace{-2em}
\end{minipage}



%We set $\alpha = 0.2$ and $\lambda_{\_T} = 0.2$ in all experiments.

\subsection{Combining Global and Local Models}
\label{sec:hybrid}
%\begin{algorithm}[!ht]
%	\caption{\golf - Deep Global Local Forecaster}
%	\label{algo:complete}
%	\small
%	\begin{algorithmic}[1]
%    \Require \texttt{maxiters}
%		%\STATE Train \MFLN model on the training data-set using Algorithm~\ref{algo:dtrmf}.
%    \State Obtain global $\*F$, $\Xtr$ and $\cT_X(\cdot)$ by Alg~\ref{algo:dtrmf}.
%    \State Obtain local \dln $\cT_Y(\cdot)$ by Alg~\ref{algo:TCtrain} on $\Ytr$.
%		\State  {/* {\em Training attention model} */ }
%    \For {$\texttt{iter} = 1,\ldots, \texttt{maxiters}$}
%      \For {each batch with indices $\cI$ and $\cJ$}
%      \State $\cI = \cbr{i_1,...,i_{b_n}}$ and $\cJ =  \cbr{s,s+1,...,s + b_t - 1}$.
%      \State Let $\hat{\*A}^{(g)},\hat{\*A}^{(l)} = \cT_A(\*Y[\cI,\cJ-1]|\Theta_A)$
%      \State $\hat{\*Y}^{(g)} = \*F[\cI,:]\*X[:, \cJ]$.
%      \State $\hat{\*Y}^{(l)} = \cT_Y(\*Y[\cI, \cJ - 1])$.
%      \State Let $\hat{\*Y} = \hat{\*Y}^{(g)}\odot\hat{\*A}^{(g)} + \hat{\*Y}^{(l)}\odot\hat{\*A}^{(l)}$
%      \State
%      $\Theta_A = \Theta_A -\eta \frac{\partial}{\Theta_A} \_L(\*Y[\_I,\cJ], \hat{\*Y})$
%      \EndFor
%		\EndFor
%	\end{algorithmic}
%\end{algorithm}
In Section~\ref{sec:trmf}, we introduced \MFLN, a model that can leverage
global information from the whole data-set even during prediction time,
through the linear combinations of the learned basis time-series. In this
section, we
will extend that model to leverage both global information (through basis
time-series in \MFLN) and local information (through a separate \dln
$\cT_Y(\cdot|\Theta_Y)$ that is trained on the original $\Ytr$ and predicts the
future values of each time-series based on its past observed values). The
final output is through a linear attention model that combines the global and
local predictions.

\begin{figure*}
	 \vspace{-1em}
	\centering

	\subfloat[][]{\includegraphics[width = 0.30\linewidth]{xnet.pdf}\label{fig:xnet}} \hfill
	\subfloat[][]{\includegraphics[width = 0.30\linewidth]{glo_illu.pdf}\label{fig:glo}} \hfill
		\subfloat[][]{\includegraphics[width = 0.30\linewidth]{scatter.png}\label{fig:scatter}}
	\caption{ \scriptsize In Fig.~\ref{fig:xnet}, we show some of the basis
  time-series extracted from the \traffic dataset, which can be combined
linearly to yield individual original time-series. It can be seen that the
basis series are highly temporal and can be predicted in the test range using
the network $\cT_X(\cdot|\Theta_X)$. Fig.~\ref{fig:glo} shows global and local predictions
on the same time-series, which are combined through $\cT_A(\cdot|\Theta_A)$,
to provide the final predictions. Note that the attention weights depend on
the time-index and adaptively combine the local and global components. In
Fig.~\ref{fig:scatter}, we display a scatter plot of the local vs global
attention weights in the test range for the time-points of all time-series in
traffic and electricity (most weights fall [0,1] therefore the range is
restricted to [0,1]). We see in that in \elec, more attention is on the
local component while in \traffic the attention is almost equal on both global
and local components.}
	\label{fig:illu}
	 \vspace{-1em}
\end{figure*}
The idea is to have a simple temporal convolution network $\cT_A$ that outputs
attention weights based on the past values of a time series $\*y^{(i)}_{s-l:s}$.
These attention weights are used to combine local and global predictions. For
The relations for one step look-ahead are as follows:
\begin{align*}
&\hat{\*X}[:,s-l+1:s+1] = \cT_X(\*X[:,s-l:s]|\Theta_X)\\
&\hat{\*Y}^{(g)}[:,s+1] = \*F\hat{\*X}[:,s+1] ~~\text{(global prediction)} \\
&\hat{\*A}^{(g)}[:,s-l+1:s+1],\hat{\*A}^{(l)}[:,s-l+1:s+1] 
=  \_T_A(\*Y[:,s-l:s])
~~\text{(attention weights)}\\
&\hat{\*Y}^{(l)}[:,s-l+1:s+1] = \_T_Y(\*Y[:,s-l:s]) ~~\text{(local pred.)}\\
&\hat{\*Y}[:,s+1] = \hat{\*Y}^{(g)}[:,s+1]\odot\hat{\*A}^{(g)}[:,s+1]+ 
 \hat{\*Y}^{(l)}[:,s+1]\odot\hat{\*A}^{(l)}[:,s+1] ~~\text{(hybrid predictions)},
\end{align*}
where $\odot$ means element-wise multiplication.

Thus the final predictions are linear combinations of the local and global
predictions. The linear attention weights,
$\hat{\*A}^{(g)}[:,s+1],\hat{\*A}^{(l)}[:,s+1]$, are predicted by a temporal
convolution network $ \cT_A(\cdot|\Theta_A)$ based on the past values of the time-series.
This network can be trained by mini-batch SGD as detailed in our complete
algorithm in Algorithm~\ref{algo:complete}. Steps 1 and 2 involve training the
global \MFLN model and the locally focused leveled network
$\cT_Y(\cdot|\Theta_Y)$ on the original $\Ytr$. Steps 6-11 is the pseudo-code
for training $\cT_A(\cdot|\Theta_A)$. 

Note that rolling predictions and multi-step predictions can be performed by
the \golf, as the individual global \MFLN model and the local \dln
$\cT_Y(\cdot|\Theta_Y)$ can perform the forecast independently, without any need for
re-training. We illustrate some representative results on a time-series from
the \elec dataset in Fig.~\ref{fig:illu}. In
Fig.~\ref{fig:xnet}, we show some of the basis time-series (global features)
extracted from the \traffic dataset, which can be combined linearly to yield
individual original time-series. It can be seen that the basis series are
highly temporal and can be predicted in the test range using the network
$\cT_X(\cdot|\Theta_X)$. Fig.~\ref{fig:glo} shows global and local predictions on the same
time-series, which are combined through $\cT_A(\cdot|\Theta_A)$, to provide
the final predictions. In Fig.~\ref{fig:scatter}, we display a scatter plot of the local
vs global attention weights in the test range for the time-points of all
time-series in \traffic and \elec (most weights fall [0,1] therefore the
range is restricted to [0,1]). We see that in \elec, more attention
is on the local component while in \traffic the attention is almost equal on
both global and local components.




